Consultation Checklists: Standardising the Human Evaluation of Medical Note Generation

Evaluating automatically generated text is generally hard due to the inherently subjective nature of many aspects of the output quality. This difficulty is compounded in automatic consultation note generation by differing opinions between medical experts both about which patient statements should be included in generated notes and about their respective importance in arriving at a diagnosis. Previous real-world evaluations of note-generation systems saw substantial disagreement between expert evaluators. In this paper we propose a protocol that aims to increase objectivity by grounding evaluations in Consultation Checklists, which are created in a preliminary step and then used as a common point of reference during quality assessment. We observed good levels of inter-annotator agreement in a first evaluation study using the protocol; further, using Consultation Checklists produced in the study as reference for automatic metrics such as ROUGE or BERTScore improves their correlation with human judgements compared to using the original human note.

==> old/02_related_work.tex <==
% \section{Related Work}
% \label{sec:related_work}
% An ideal evaluation protocol would minimise the subjectivity of the task, but still provide insights into the generation system errors.
% There are a number of different approaches to human evaluation in NLG:

% % varying in how much insight the results provide; how subjective the evaluation task is, measured by inter-annotator agreement; and how cost-effective it is in resources, time and cognitive load.
% \begin{enumerate}[leftmargin=*]
%     \itemsep0em
%     \item 
%     Ranking texts according to how `good' they are \cite{zhang2018learning, zhang2020optimizing, joshi2020dr} is fast but does not provide any insights about what type of errors the NLG systems make and how to improve them.
    
%     \item Rating scales work well for a few criteria but again are not very insightful. With many criteria, they become more useful but also more expensive and cumbersome; e.g. \citet{MOEN201625} use 30 items (Long-term diagnoses, Reason for admission, Assessment of the future, etc.) with a rating scale each (not relevant, not included, partially included and fully included) and report that subjects found the 30 item scale too difficult and detailed to assess.
    
%     \item Measuring post-edit time \cite{moramarco2022human} provides an extrinsic measure of how useful the generated text may be to the final user, but it’s expensive, subjective \cite{lai2022exploration}, and again does not provide insights into the system errors. 
    
%     \item Extracting errors and listing omissions \cite{moramarco2022human} help quantify the factual accuracy and the completeness of the NLG system, but it’s more expensive still and even though the evaluators are usually experts (medical practitioners), agreement is very low.
    
% \end{enumerate}
% % An ideal evaluation protocol would minimise the subjectivity of the task, but still provide insights into the generation system errors. The evaluation method in \citet{moramarco2022human} does provide the required insight, but reported agreement is low.
% While the agreement in \citet{moramarco2022human} could be improved by better evaluator training, we believe that the evaluation task itself inherently inhibits agreement: the evaluators are asked to listen to the recording of a consultation, then identify the number of missing and incorrect statements in a generated note. However, both the total number of statements in a consultation and the total number of statements in a given generated note are subjective and differ between evaluators.
% In other words, the “ground truth” for this task, the recording of the consultation, is implicit rather than explicit; thus open to evaluator interpretation. This makes it very hard to align multiple evaluators and get consistent results.



==> old/05_generated_notes.tex <==


% \section{System-generated Notes}
% \label{sec:generated-notes}

% The system-generated notes discussed in this paper were produced with two BART \cite{lewis2020bart} encoder-decoder transformer models\footnote{\url{https://huggingface.co/facebook/bart-large-cnn}} pre-trained on the CNN/Dailymail dataset [cite] and fine-tuned on a proprietary dataset of 10,000 real consultations. The input to the models was the transcript of the consultation recording (automatically produced with Google Speech-to-text) and the output was the History and Examination parts of the note written by the consulting clinician.\footnote{The only difference between the two models is that one of them encodes the patient gender as an explicit input, but this is unrelated to the purpose of this study.}


% For the purpose of the human evaluation, the system-generated notes were split into statements in a way that mimics the Checklists. However, this was done automatically by splitting in sentences and then on commas, ‘and’, and ‘but’. The first statement in each sentence is considered a top level statement and all others are items in a sublist (column E in Figure \ref{fig:note-evaluation}). We instruct evaluators to read the full sentence before marking each statement as they may be meaningless in isolation.
